Scale-Aware Dynamic Network for Continuous-Scale Super-Resolution

Single-image super-resolution (SR) with fixed and discrete scale factors has achieved great progress due to the development of deep learning technology. However, the continuous-scale SR, which aims to use a single model to process arbitrary (integer or non-integer) scale factors, is still a challenging task. The existing SR models generally adopt static convolution to extract features, and thus unable to effectively perceive the change of scale factor, resulting in limited generalization performance on multi-scale SR tasks. Moreover, the existing continuous-scale upsampling modules do not make full use of multi-scale features and face problems such as checkerboard artifacts in the SR results and high computational complexity. To address the above problems, we propose a scale-aware dynamic network (SADN) for continuous-scale SR. First, we propose a scale-aware dynamic convolutional (SAD-Conv) layer for the feature learning of multiple SR tasks with various scales. The SAD-Conv layer can adaptively adjust the attention weights of multiple convolution kernels based on the scale factor, which enhances the expressive power of the model with a negligible extra computational cost. Second, we devise a continuous-scale upsampling module (CSUM) with the multi-bilinear local implicit function (MBLIF) for any-scale upsampling. The CSUM constructs multiple feature spaces with gradually increasing scales to approximate the continuous feature representation of an image, and then the MBLIF makes full use of multi-scale features to map arbitrary coordinates to RGB values in high-resolution space. We evaluate our SADN using various benchmarks. The experimental results show that the CSUM can replace the previous fixed-scale upsampling layers and obtain a continuous-scale SR network while maintaining performance. Our SADN uses much fewer parameters and outperforms the state-of-the-art SR methods.

==> sections/__latexindent_temp.tex <==
\section{Experiments}

In this section, we first introduce the datasets, metrics, and training details. Then, we compare our model with the SOTA continuous scale and fixed scale SR methods. Finally, we investigate the effectiveness of each component through ablation experiments.

\input{tables/1-scale-arbitrary-results.tex}

\subsection{Datasets and Metrics}
We use DIV2K\cite{agustsson2017ntire} containing 800 high-resolution images as our training dataset. For testing, we evaluate SR models on five standard benchmark datasets: Set5\cite{bevilacqua2012low}, Set14\cite{zeyde2010single}, B100\cite{martin2001database}, Manga109\cite{matsui2017sketch}, and Urban100\cite{huang2015single}. Following the settings of previous works, we only consider the PSNR and SSIM\cite{wang2004image} of the Y channel of the transformed YCbCr space. Following previous works, we use bicubic downsampling as the standard degradation model for generating LR images from their HR counterparts.

\input{tables/2-scale-fixed-results.tex}

\subsection{Training Details}
In the training phase, we randomly crop LR patches with a size of $48\times 48$ as input. We randomly flip images vertically or horizontally and randomly rote them $90^{\circ}$ for data augmentation. We train our model for 1000 epochs with a mini-batch size of 16, and each epoch contains 1000 iterations. The initial learning is $1\times 10^{-4}$ and decreases by half every 200 epochs. The scale factors of each batch of images are the same, and the scale factors in the training phase are uniformly distributed from 1 to 4. Our model is implemented using the PyTorch framework and trained on an Nvidia GeForce RTX 3090 GPU.

\subsection{Comparison with Continuous-Scale SR Methods}
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.95\textwidth]{imgs/mainrslt_Set14_x26.pdf}
  \vspace{5pt}\\
  \includegraphics[width=0.95\textwidth]{imgs/mainrslt_BSD100_x39.pdf}
  \caption{Visual comparisons between continuous-scale SR methods. The top two rows are results with a scale factor of $\times 2.6$ and the bottom two rows are results with a scale factor of $\times 3.9$.}
  \label{fig:mainrslt_Set14_x26}
\end{figure*}

\begin{figure*}[tbp]
  \centering
  \includegraphics[width=0.95\linewidth]{imgs/mainrslt_Urban100_x8.pdf}
  \vspace{5pt}\\
  \includegraphics[width=0.95\linewidth]{imgs/mainrslt_Manga109_x10.pdf}
  \caption{Visual comparisons with out-of-distribution integer scale factors. The top two rows are results with a scale factor of $\times 8$ and the bottom two rows are results with a scale factor of $\times 10$.}
  \label{fig:mainrslt_large_scale}
\end{figure*}

\begin{figure*}[tbp]
  \centering
  \includegraphics[width=0.95\linewidth]{imgs/mainrslt_Set14_x2.pdf}
  \vspace{5pt}\\
  \includegraphics[width=0.95\linewidth]{imgs/mainrslt_Urban100_x3.pdf}
  \vspace{5pt}\\
  \includegraphics[width=0.95\linewidth]{imgs/mainrslt_Urban100_x4.pdf}
  \caption{Visual comparisons between SOTA fixed-scale and continuous-scale SR methods. The top two rows are results with a scale factor of $\times$2, the middle two rows are results with a scale factor of $\times$3 and the bottom two rows are results with a scale factor of $\times$4.}
  \label{fig:mainrslt_integer_scales}
\end{figure*}

We take bicubic interpolation as the baseline and compare our proposed CSUM with three continuous-scale upsampling modules. The meta-upsampling module proposed in MetaSR \cite{Hu2019} is a pioneering method for arbitrary-scale upsampling. The LIIF \cite{chen2021learning} is an SOTA continuous-scale SR method based on implicit functions. The OSM \cite{behjati2021overnet}, based on overscaling and interpolation, can achieve any scale SR within a certain range. For a fair comparison, we replace the original upsampling layer of EDSR-baseline (EDSR-B) \cite{Lim2017} and the RDN \cite{Zhang2018d} with the OSM, the meta-upsampling module, the LIIF, and our proposed CSUM. Therefore, we obtain six different model combinations, namely, OSM-EDSR-B, Meta-EDSR-B, LIIF-EDSR-B, CSUM-EDSR-B, OSM-RDN, Meta-RDN, LIIF-RDN, and CSUM-RDN. Besides, we define a new baseline by resampling the output of a fixed-scale SR model to the target size. Specifically, we adopt the RDN model with a fixed scaling factor of $\times$4. For scaling factor $r$, the input LR image is first upscaled by the RDN model and then resampled by bicubic interpolation with a scale factor of $r/4$. This baseline is called the Bi-RDN. We also add our proposed SADN and the lightweight version SADN-L for comparison.

The results of the OSM and MetaSR are from our implementation, and the results of the LIIF are obtained by using the official code and pre-trained models. The CSUM-EDSR and CSUM-RDN are retrained from scratch. In addition to the scale factors in the training distribution ($\times 1$ -- $\times$4), we also evaluate models on large-scale factors out of the training distribution to test the generalization performance. The quantitative results are shown in Table\,\ref{tab:scale-arbitrary-results}. The best results of all comparisons are bolded, and the second best results are underlined.

As the table shows, our proposed CSUM-EDSR-B obtains the best results among all EDSR-B-based methods, and CSUM-RDN obtains the best results among all RDN-based methods. In particular, the proposed CSUM has made significant progress on small scale factors, such as an increase of $0.25$ dB with a scale factor $\times 1.1$. The performance of CSUM-EDSR-B and CSUM-RDN demonstrates that the proposed CSUM can replace the upsampling layer of previous SR networks and obtain satisfactory results. Moreover, benefiting from the scale-aware feature extractor, our proposed SADN obtains the best object metrics on almost all scale factors.

We compare the visual results of the continuous-scale SR methods in Fig.\,\ref{fig:mainrslt_Set14_x26}. Furthermore, Fig.\,\ref{fig:mainrslt_large_scale} shows the visual comparisons of large-scale factors out of the training distribution. Our proposed SADN performs better at restoring clear details and sharp edges. Besides, CSUM-EDSR-B and CSUM-RDN obtain more convincing results among all EDSR-B-based and RDN-based methods, respectively. In summary, our proposed upsampling module combined with the scale-aware feature extractor can achieve better visual performance.

\subsection{Comparison with the SOTA Methods}

We compare our proposed SADN with SOTA fixed-scale SR methods, including CFSRCNN \cite{tian2020coarse}, SRFBN \cite{Li2019c}, RDN \cite{Zhang2018d}, ISNR \cite{liu2021iterative}, and SAN \cite{dai2019second}; and continuous-scale SR methods, including OverNet \cite{behjati2021overnet}, Meta-RDN \cite{Hu2019} and LIIF-RDN \cite{chen2021learning}, on five benchmark datasets. The results of RDN, SRFBN, and SAN are obtained by retraining on each scale factor. The results of the continuous-scale comparative methods are obtained using a single model without fine-tuning. We also use the self-ensemble \cite{timofte2016seven} strategy to further improve the performance of the SADN, and the method is named SADN+.

Table\,\ref{tab:scale-fixed-results} shows the quantitative results with scale factors of $\times$2, $\times$3, and $\times$4. Our proposed SADN achieves the best performance on most datasets and scales. The results demonstrate that our proposed SADN has made great progress compared to the existing continuous-scale SR methods and obtains comparable and even better results with the SOTA fixed-scale methods, such as the SAN. Compared with the lightweight networks CFSRCNN and OverNet, our SADN-L also performs better on objective metrics. Thanks to the CSUM, our proposed SADN and SADN-L only need to be trained once and save a single model while the fixed-scale methods need to be trained several times and save a model for each scale factor. Therefore, the SADN not only greatly saves training time and model storage space compared to fixed-scale SR models but also bridges the performance gap between the continuous-scale SR models and the fixed-scale SR models.

Fig.\,\ref{fig:mainrslt_integer_scales} shows the visual results with scale factors of $\times$2, $\times$3, and $\times$4. In general, the SADN can obtain more realistic SR images. For the SR results of ``ppt3'' from Set14, our SADN can clearly recover all letters, especially the letter ``i'' and the letter ``t''. For ``img\_004'' from Urban100, the proposed SADN produces circles that are very close to the ground truth. The good visual results are attributable to the fact that our proposed SADN makes full use of multi-level features and a larger range of latent codes to achieve reconstruction, so more realistic SR images can be obtained at different scales. In addition, scale-aware feature extraction also ensures that good results can be obtained at multiple scale factors.

\subsection{Network Parameters}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{imgs/parameter.pdf}
  \caption{Performance vs. number of parameters. The results are evaluated on the Set14 dataset with a scale factor of $\times$3. The red points represent our proposed networks.}
  \label{fig:parameter}
  \vspace{-0.5em}
\end{figure}

We compare the network parameters and model performance of our proposed SADN with nine comparative methods, including LapSRN\cite{Lai2017deep}, MemNet\cite{tai2017memnet}, OverNet\cite{behjati2021overnet}, SRFBN\cite{Li2019c}, RCAN\cite{zhang2018image}, SAN\cite{dai2019second}, RDN\cite{Zhang2018d}, LIIF-RDN \cite{chen2021learning}, and Meta-RDN \cite{Hu2019}. The comparison results are shown in Fig.\,\ref{fig:parameter}.

The proposed SADN achieves the best performance and uses only 7.6\,M parameters, which is 1/3 of the number of parameters of MetaSR and LIIF. Furthermore, our proposed lightweight model SADN-L has fewer than 1\,M parameters, and it outperforms OverNet with 1.7\,M parameters. Thanks to the feedback structure, our method can balance the number of network parameters and model performance well.

\begin{table}[t]
  \caption{Average Running Time Comparison on Set14 Dataset with a Scale Factor of $\times$4 on an NVIDIA 3090 GPU.  * Indicates Our Proposals.}
  \renewcommand\arraystretch{0.9}
  \centering
  \begin{tabular}{|l|ccc|}
    \hline
    Method                            & \multicolumn{1}{l}{Parameters (M)} & \multicolumn{1}{l}{Running Time (s)} & \multicolumn{1}{l|}{PSNR (dB)} \bigstrut \\
    \hline\hline
    OverNet \cite{behjati2021overnet} & 1.7                                & 0.0173                               & 28.65 \bigstrut[t]                       \\
    SADN-L*                           & 1.0                                & 0.0232                               & 28.72                                    \\
    RDN \cite{Zhang2018d}             & 22.3                               & 0.0426                               & 28.81                                    \\
    CSUM-RDN*                         & 22.7                               & 0.0628                               & 28.82                                    \\
    Meta-RDN \cite{Hu2019}            & 22.4                               & 0.0666                               & 28.77                                    \\
    SADN*                             & 7.6                                & 0.0881                               & 28.91                                    \\
    SAN \cite{dai2019second}          & 15.9                               & 0.1118                               & 28.92                                    \\
    LIIF-RDN \cite{chen2021learning}  & 22.3                               & 0.1508                               & 28.80                                    \\
    SRFBN \cite{Li2019c}              & 4.0                                & 0.3324                               & 28.81  \bigstrut[b]                      \\
    \hline
  \end{tabular}%
  \label{tab:runtime}
\end{table}

\subsection{Running Time}
We compare the running time of our proposed methods with six methods, OverNet \cite{behjati2021overnet}, RDN \cite{Zhang2018d}, Meta-RDN \cite{Hu2019}, SAN \cite{dai2019second}, LIIF-RDN \cite{chen2021learning}, and SRFBN \cite{Li2019c}, on the Set14 dataset with a scale factor of $\times$4. The running time of all comparative methods is evaluated on an NVIDIA 3090 GPU. The comparison results are shown in Table\,\ref{tab:runtime}.

First, comparing the CSUM-RDN, Meta-RDN, and LIIF-RDN, we find that the CSUM has a running time that is only $0.02\,\mathrm{s}$ longer than that of the baseline RDN method while the LIIF takes $0.11\,\mathrm{s}$ longer. The results demonstrate that our proposed CSUM is a highly efficient upsampling module that runs 5.5$\times$ faster than the LIIF on the Set14 dataset. Moreover, compared to the SOTA SAN, our proposed SADN runs 1.3$\times$ faster and achieves comparable performance. The results show that our proposed SAFL part can extract powerful high-level features with low computational costs.

\section{Discussion}
In this section, we first investigate the random scale training strategy. Then, we present ablation studies of the feature extractor and the CSUM. Finally, we investigate the parameter settings.

\subsection{Training with a Single Scale} To investigate the differences and relationships between the SR tasks of various scale factors, below, we test the generalization performance of a model trained on a single scale factor. We train the proposed SADN with three single scales ($\times $2, $\times $3, and $\times $4) and obtain three models, named SADN-x2-only, SADN-x3-only, and SADN-x4-only, respectively. Then, the three models are tested across scales. We compare the three models with the SADN, which is trained with randomly sampled scale factors.

Fig.\,\ref{fig:cross_scale} shows the comparison results. We have two observations. First, the model trained with a single scale factor can only obtain satisfactory results on the trained scale factor while the SADN obtains the best performance on all scale factors. This observation indicates that there are essential differences between SR tasks with various scale factors. Our uniform distribution training strategy can significantly improve the performance of multi-scale SR tasks. Thanks to the scale-aware strategy, our proposed continuous-scale SR model can adapt to multiple learning tasks well. Second, training with a single large-scale factor can also boost the performance on other scale factors, and the model trained on a large-scale factor has better generalization performance. This result shows that there are similarities between SR tasks with various scale factors, and it is reasonable to use a unified framework to process these multi-scale tasks.

\begin{figure}[tbp]
  \centering
  \includegraphics[width=0.8\linewidth]{imgs/cross_scale.pdf}
  \caption{Investigation of the generalization performance across scales.}
  \label{fig:cross_scale}
  \vspace{-1em}
\end{figure}

\subsection{Feature Extractor Ablation Study} First, to investigate the effectiveness of the scale-aware feature learning strategy, we replace SAD-Conv with a common convolutional layer with the same kernel size. Thus, a feature learning module without the scale-aware strategy is obtained. To show the difference between the SAD-Conv and the common convolutional layer, we visualize the average feature maps with different scale factors output by the SAFL modules with and without the SAD-Conv, as shown in Fig.\,\ref{fig:ablation_saconv}. We find that thanks to SAD-Conv, the SAFL can learn different feature representations based on the input scale factor while the common convolutional counterpart outputs the same feature maps for all scale factors.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{imgs/ablation_saconv.pdf}
  \caption{Average feature maps output by the SAFL modules with and without SAD-Conv. }
  \label{fig:ablation_saconv}
\end{figure}

Second, to explore the influence of the feedback strategy, we design a feedforward feature learning counterpart by removing all the feedback connections. Compared with the SAFL, the feedforward feature learning part only lacks a few $1\times 1$ convolutional layers for fusing the feedback features, and the number of parameters is almost the same. In this case, the feature extractor can only output one level of features as in the previous methods.

Table \ref{tab:feature_extrator_ablation} shows the PSNR comparison of different ablation models. It is observed that both the SAD-Conv and feedback strategy can improve SR performance independently. This result can be attributed to the following two aspects. First, the dynamic convolution module can provide stronger feature extraction capabilities for multi-task (multi-scale SR) learning. Second, the feedback strategy makes it possible that smaller-scale features are computed with fewer iterations while higher-scale features are refined several times from multiple recurrences. Therefore, by continuously correcting low-level features, more accurate latent codes are provided for the implicit functions, thereby improving the SR performance.

\begin{table}[tb]
  \centering
  \caption{Ablation Study on SAD-Conv and Feedback Strategy. The Models use the Same Parameters as SADN-L. The Average PSNR({\rm dB}) values are Evaluated on Set14 in $400$ Epochs.}
  \renewcommand\arraystretch{0.9}
  \begin{tabular}{|cc|rrrrr|}
    \hline
    \multicolumn{1}{|l}{SAD-Conv} & \multicolumn{1}{l|}{Feedback} & \multicolumn{1}{c}{$\times$2} & \multicolumn{1}{c}{$\times$3} & \multicolumn{1}{c}{$\times$4} & \multicolumn{1}{c}{$\times$6} & \multicolumn{1}{c|}{$\times$8} \bigstrut \\
    \hline
    \hline
    $\bm\times$                   & $\bm\times$                   & 33.29                         & 30.09                         & 28.38                         & 26.24                         & 27.74 \bigstrut[t]                       \\
    $\checkmark$                  & $\bm\times$                   & 33.38                         & 30.18                         & 28.48                         & 26.28                         & 24.78                                    \\
    $\bm\times$                   & $\checkmark$                  & 33.43                         & 30.20                         & 28.49                         & 26.26                         & 24.84                                    \\
    $\checkmark$                  & $\checkmark$                  & \textbf{33.53}                & \textbf{30.28}                & \textbf{28.55}                & \textbf{26.37}                & \textbf{24.85}\bigstrut[b]               \\
    \hline
  \end{tabular}%   
  \label{tab:feature_extrator_ablation}
\end{table}

\subsection{CSUM Ablation Study}
\label{sec:CSUM_ablation}
First, we investigate the choices of local implicit feature functions in the CSUM. One of the simplest choices is to directly use the latent code with the nearest Euclidean distance as the feature of the query point. The CSUM thus defined is called CSUM-Nearest. We also use a learning-based local implicit feature function to construct the CSUM, where the local implicit feature function is a 2-layer MLP. The MLP takes the latent code set and query coordinates as input and outputs a feature vector of the query point. The CSUM thus defined is called CSUM-MLP.

Second, we investigate the scale-aware feature fusion strategy in the MBLIF. We build a CSUM without the scale-aware attention block, named CSUM-w/o-SA, in which the feature weights of all levels are the same regardless of the scale factor.

The results are shown in Table\,\ref{tab:csum_ablation}. The table shows that only using the nearest neighbor latent code to construct the MBLIF will degrade performance. Although the local implicit feature function based on the MLP seems to be more flexible, it also brings learning difficulties, resulting in a decrease in model performance. Thus, we choose the parameter-free bilinear functions to construct the MBLIF because of its high computational efficiency and effectiveness. In addition, we found that the scale-aware feature fusion strategy helps to improve SR performance.

\begin{table}[t]
  \centering
  \caption{Ablation Study on Different Choices of CSUM. The Feature Extractor of all Models is EDSR-B. The Average PSNR({\rm dB}) values are Evaluated on Set14 in $400$ Epochs.}
  \renewcommand\arraystretch{0.9}
  \begin{tabular}{|l|rrrrr|}
    \hline
    Choices of CSUM & \multicolumn{1}{c}{$\times$2} & \multicolumn{1}{c}{$\times$3} & \multicolumn{1}{c}{$\times$4} & \multicolumn{1}{c}{$\times$6} & \multicolumn{1}{c|}{$\times$8} \bigstrut \\
    \hline
    \hline
    CSUM-Nearest    & 32.88                         & 30.01                         & 27.91                         & 26.01                         & 24.09 \bigstrut[t]                       \\
    CSUM-MLP        & 33.41                         & 30.21                         & 28.48                         & 26.32                         & 24.78                                    \\
    CSUM-w/o-SA     & 33.39                         & 30.14                         & 28.47                         & 26.24                         & 24.70                                    \\
    CSUM            & \textbf{33.51}                & \textbf{30.29}                & \textbf{28.54}                & \textbf{26.38}                & \textbf{24.84} \bigstrut[b]              \\
    \hline
  \end{tabular}%
  \label{tab:csum_ablation}
\end{table}

\subsection{Number of Scales in the CSUM}

We investigate the number of scales $T$ in the CSUM. Because the number of iterations of the proposed SAFL needs to be the same as $T$ in the CSUM, to eliminate the effect of the feature learning part when $T$ changes, we take EDSR-B as the feature extractor in this investigation. Fig.\,\ref{fig:levels} shows that the performance continues to improve as $T$ increases from 1 to 4. This result demonstrates that using multi-scale features to construct implicit functions can significantly improve the reconstruction quality compared to using only single-scale features. In other words, our CSUM surely benefits from the multi-scale features. Although choosing a large $T$ contributes to better results, it will exponentially increase the size of the input feature maps of the MBLIF and may result in out of GPU memory. Therefore, we comprehensively weigh the performance and computational burden and set $T$ to 4 and 3 in the SADN and SADN-L, respectively.

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.85\linewidth]{imgs/levels.pdf}
  \caption{Investigation of the number of scales in the CSUM. Models are evaluated on Set14 over 400 epochs.}
  \label{fig:levels}
  \vspace{-1em}
\end{figure}

\begin{table}[tb]
  \centering
  \renewcommand\arraystretch{0.9}
  \caption{Investigation of the number of kernels in SAD-Conv. The Average PSNR({\rm dB}) values are Evaluated on Set14 in $400$ Epochs.}
  \begin{tabular}{|l|ccccc|}
    \hline
    \multicolumn{1}{|c|}{Models} & $\times$2      & $\times$3      & $\times$4      & $\times$6      & $\times$8 \bigstrut         \\
    \hline
    \hline
    SADN-L (K=1)                 & 33.43          & 30.20          & 28.49          & 26.26          & 24.84  \bigstrut[t]         \\
    SADN-L (K=2)                 & 33.50          & 30.25          & 28.53          & 26.32          & 24.84                       \\
    SADN-L (K=3)                 & \textbf{33.53} & \textbf{30.28} & \textbf{28.55} & \textbf{26.37} & 24.85                       \\
    SADN-L (K=4)                 & 33.51          & 30.26          & 28.52          & 26.36          & \textbf{24.86} \bigstrut[b] \\
    \hline
  \end{tabular}%
  \label{tab:ablation_K}%
\end{table}

\subsection{Number of Kernels in SAD-Conv} We investigate the number of kernels $K$ in SAD-Conv. Table\,\ref{tab:ablation_K} shows the PSNRs for SAD-Conv with different $K$s. Firstly, the SAD-Conv with $K>1$ outperforms its static convolution counterpart ($K=1$) for all scale factors. Even using a small $K=2$ can significantly increase performance. This demonstrates the strength of our dynamic feature learning strategy. Second, the PSNRs stop increasing once $K$ is larger than 3. Although the representation power of the model enhances as $K$ increases, it is more difficult to learn all kernels and corresponding attention weights simultaneously, and the network is more difficult to converge.


\subsection{Investigation of Parameters Settings} We explore the settings of the key hyperparameters in the SAFL part, including the number of LDGs $D$ in each iteration and the number of SARBs $C$ in an LDG. We fix $C=4$ and let $D$ vary from 2 to 4. Besides, we study the influence of $C$ by fixing $D$ to 4. The results are presented in Fig.\,\ref{fig:ablation_parameter}. The figure shows that a larger $C$ and $D$ lead to better performance because a deeper network has a stronger representation ability.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{imgs/ablation_parameter.pdf}
  \caption{Investigation of $C$ and $D$. the models are evaluated on Set14 with a scale factor of $\times$2 over 400 epochs.}
  \label{fig:ablation_parameter}
  \vspace{-1em}
\end{figure}

